A Spatiotemporal Model for Peak AoI in Uplink IoT Networks: Time Vs Event-triggered Traffic

Timely message delivery is a key enabler for Internet of Things (IoT) and cyber-physical systems to support wide range of context-dependent applications. Conventional time-related metrics (e.g. delay and jitter) fails to characterize the timeliness of the system update. Age of information (AoI) is a time-evolving metric that accounts for the packet inter-arrival and waiting times to assess the freshness of information. In the foreseen large-scale IoT networks, mutual interference imposes a delicate relation between traffic generation patterns and transmission delays. To this end, we provide a spatiotemporal framework that captures the peak AoI (PAoI) for large scale IoT uplink network under time-triggered (TT) and event triggered (ET) traffic. Tools from stochastic geometry and queueing theory are utilized to account for the macroscopic and microscopic network scales. Simulations are conducted to validate the proposed mathematical framework and assess the effect of traffic load on PAoI. The results unveil a counter-intuitive superiority of the ET traffic over the TT in terms of PAoI, which is due to the involved temporal interference correlations. Insights regarding the network stability frontiers and the location-dependent performance are presented. Key design recommendations regarding the traffic load and decoding thresholds are highlighted.

==> QT_anaylsis/figures/DTMC_diagram/1col/DTMC_diagram.tex <==

\begin{tikzpicture}
\begin{groupplot}[group style={
	group size= 1 by 2, vertical sep=1cm},height=3.45in, width=3.45in]
\nextgroupplot[title={{(a)}}]
	\input{QT_anaylsis/figures/DTMC_diagram/2col/DTMC_diagram_P.tex}
\nextgroupplot[title={{\smash{(b)}}}]
	\input{QT_anaylsis/figures/DTMC_diagram/2col/DTMC_diagram_P.tex}
\end{groupplot}

\end{tikzpicture}

==> QT_anaylsis/figures/DTMC_diagram/2col/DTMC_diagram.tex <==

\begin{tikzpicture}
\begin{groupplot}[group style={
	group size= 1 by 2, vertical sep=1cm},height=3.45in, width=3.45in]
\nextgroupplot[title={{(a)}}]
	\input{QT_anaylsis/figures/DTMC_diagram/2col/DTMC_diagram_P.tex}
\nextgroupplot[title={{\smash{(b)}}}]
	\input{QT_anaylsis/figures/DTMC_diagram/2col/DTMC_diagram_P.tex}
\end{groupplot}

\end{tikzpicture}

==> simulation_results/figures/AoI_Arrival/AoI_Arrival.tex <==
\definecolor{mycolor1}{rgb}{1.00000,0.00000,1.00000}%

\begin{tikzpicture}[scale=0.9]
\begin{groupplot}[group style={
	group name=myplot2,
	group size= 1 by 2, , vertical sep=1.8cm}, height=2in,width=3in]

\nextgroupplot[title={{(a) Periodic traffic}},
scale only axis,
xmin=0,
xmax=1,
xlabel={$\xi$},
ymin=0,
ymax=1,
ylabel={$\bar{F}_B(\theta, \xi)$},
xtick={0,0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9,1},
grid=both,
legend style={at={(0.1,-0.4)},legend columns=2, anchor=south west, legend cell align=left, align=left,column sep=0.13cm}]



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nextgroupplot[title={{(b) Bernoulli traffic}},
scale only axis,
xmin=0,
xmax=1,
xlabel={$\xi$},
ymin=0,
ymax=1,
ylabel={$\bar{F}_B(\theta, \xi)$},
xtick={0,0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9,1},
grid=both,
legend style={at={(0.1,-0.4)},legend columns=2, anchor=south west, legend cell align=left, align=left,column sep=0.13cm}]


\end{groupplot}


\end{tikzpicture}
